UniAdapt: A Universal Adapter for Knowledge Calibration

Large Language Models (LLMs) require frequent updates to correct errors and keep pace with continuously evolving knowledge in a timely and effective manner. Recent research in it model editing has highlighted the challenges in balancing generalization and locality, especially in the context of lifelong model editing. We discover that inserting knowledge directly into the model often causes conflicts and potentially disrupts other unrelated pre-trained knowledge. To address this problem, we introduce UniAdapt, a universal adapter for knowledge calibration. Inspired by the Mixture of Experts architecture and Retrieval-Augmented Generation, UniAdapt is designed with a vector-assisted router that is responsible for routing inputs to appropriate experts. The router maintains a vector store, including multiple shards, to construct routing vectors based on semantic similarity search results. UniAdapt is fully model-agnostic and designed for seamless plug-and-play integration. Experimental results show that UniAdapt outperforms existing lifelong model editors and achieves exceptional results in most metrics.

==> _analysis.tex <==
\section{Results and Analyses}

\subsection{Ablation Study}

% \noindent\textbf{Routing Strategy}: The performance of \tool~heavily depends on the performance of the router. Thus, we perform a set of experiments to study how well our proposed router in the classification problem.

% \noindent\textbf{Single Editing vs Sequential Editing}: We progressively increase the number of edits from 1 to 1000

\begin{figure}[h!]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/target_layer.png}
        % \caption{Caption for figure 1}
        \label{fig:figure1}
    \end{minipage}\hfill
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/noe.pdf}
        % \caption{Caption for figure 2}
        \label{fig:figure2}
    \end{minipage}
    \caption{LLaMA2-7b, Counterfact, seq=True}
\end{figure}

\noindent\textbf{Effect of Expert Number}. We perform a set of experiments to study how does number of experts impact the performance. Figure~XXX illustrates the performance of \tool~with different numbers of experts. Due to computational resource limitations, we sequentially set the number of experts to $\{1, 2, 4, 8\}$ and evaluate our edits after 1000 edits. We find that the reliability and locality of model editing do not change with the number of experts; there is neither a decrease nor an improvement in performance. However, the generalization of knowledge fluctuated with the
number of experts, peaking when the number of experts is XXX. We hypothesize that this optimal experts number is related to the difficulty of the dataset. If it is easy to distinguish between rephrased fact and unrelated fact then the number of experts does not affect much on the performance. In contrast, it requires more experts to store new knowledge.
